Registration Techniques for Deformable Objects

In general, the problem of non-rigid registration is about matching two different scans of a dynamic object taken at two different points in time. These scans can undergo both rigid motions and non-rigid deformations. Since new parts of the model may come into view and other parts get occluded in between two scans, the region of overlap is a subset of both scans. In the most general setting, no prior template shape is given and no markers or explicit feature point correspondences are available. So, this case is a partial matching problem that takes into account the assumption that consequent scans undergo small deformations while having a significant amount of overlapping area [28]. The problem which this thesis is addressing is mapping deforming objects and localizing cameras in the environment at the same time.

==> parts/conclusion.tex <==
% !TEX root = ../thesis.tex

%\lettrine{S}{tart} with the text that basically says the same things as
%abstract, but not in the same workds. It is a short summary of your work stating
%why it is so important and what problems does it solve exactly.
\lettrine{R}{obotic} agents are being used frequently in more complex roles in our life, nowadays. One of the requirement for them to perform with their tasks is to have a robust perception of the environment. In Robotics this problem is often studied under the title  Simultaneous Localization and Mapping (SLAM). SLAM enables robots to build a map of the environment while exploring in it and at the same time localize itself. Often the environment around the robots is not static, forcing researchers to look for a way to deal with dynamic environments to construct consistent maps. 

In this thesis, we aim to address the task of 3D mapping of scenes with both static and deformable objects. We presented an approach that integrates RGB-D scans into a dense volumetric representation which works well for statics scenes. Furthermore, we have proposed a method that captures the non-rigidity of the scene, which the regular rigid SLAM pipeline can not handle. The proposed extended pipeline can deal with dynamic environments and reconstruct models of deformable objects. We tested our approach on synthetic data, and developed algorithms to work online on the robotic platforms.


\section{Short summary of key contributions}

In this thesis, we studied the problem of mapping rigid and non-rigid object using RGB-D sensors. We proposed solutions to several challenges in dense non-rigid SLAM problem. We have inferred our approach from the state of-the-art non-rigid mapping literatures \cite{newcombe2015dynamicfusion}, \cite{innmann2016volumedeform}. The main contributions of this thesis are briefly mentioned in the following:
\begin{itemize}
	\item A method to construct a dense volumetric representation of the environment using geometric and photometric information of the scene along with the tracking camera pose in the real-time. The proposed technique is based on $KinectFusion$ \cite{izadi2011kinectfusion} and voxel hashing technique \cite{niessner2013real}. The results of this part shows, our approach is able to track camera pose while having harsh motions and construct volumetric model of the surroundings in real-time with fine details and deal with noisy inputs. 
	
	\item A novel approach to integrate the non-rigidity to regular mapping systems which enables them to reconstruct 3D models from deforming objects based on RGB-D scans. Our method is inspired from deformation graph idea ~\cite{sumner2007embedded} and $DynamicFusion$ ~\cite{newcombe2015dynamicfusion}, which enables us to map non-rigid scenes. The proposed approach is tested via synthetic data and is able to estimate and warp deformations between two surfaces efficiently. 
	
\end{itemize}

\section{Open source contributions} % (fold)
\label{sec:open_source_contributions}

The implementation of presented thesis is released as an open-source software and belonging developed libraries are publicly published and listed below:

\url{https://github.com/alirezaahmadi/dynamap}

\begin{enumerate}
	\item CUDA Compatible DynaMap image processing library including  (Convolution, Kernel Generation, Bilateral filter, Gaussian Filter, Pyramid image scaling, normal extraction,  ...).
	\item Quaternion and Dual-Quaternion libraries compatible with CUDA
	\item TSDF (Volumetric representation of environment)
	\item OpenGL based GUI
	\item Accelerated marching cubes
	\item Accelerated Ray-tracing (Mesh-to-RGB-D)
	\item CUDA compatible implementation of Deformation Graph 
	\item Rigid and non-rigid tracking pipeline on CPU and GPU (using cuSolver, Eigen libraries)
	\item KDTree 
	\item Loading datasets and evaluation tools
\end{enumerate}

all mentioned libraries are released under the address of :

\url{https://github.com/alirezaahmadi}

\section{Future Work}
In this thesis, we presented our mapping firmware which can densely map rigid environments. Also, we have tried to develop a state-of-the-art method to introduce the non-rigidity into the conventional SLAM system which can estimate and warp deformations in the target scans. Our firmware is able to work properly on synthetic data, while the whole requirements and pipe-line are developed to work on dense scans, as well. Despite the discussed progress, there are still many difficult open challenges that future work on non-rigid 3D reconstruction with RGB-D cameras needs to address, in particular for online reconstructions and in the case with a highly dynamic target. 
